AI-augmented Automation for Real Driving Prediction: an Industrial Use Case

The risen complexity of automotive systems requires new development strategies and methods to master the upcoming challenges. Traditional methods need thus to be changed by an increased level of automation, and a faster continuous improvement cycle. In this context, current vehicle performance tests represent a very time-consuming and expensive task due to the need to perform the tests in real driving conditions. As a consequence, agile/iterative processes like DevOps are largely hindered by the necessity of triggering frequent tests. This paper reports on a practical experience of developing an AI-augmented solution based on Machine Learning and Model-based Engineering to support continuous vehicle development and testing. In particular, historical data collected in real driving conditions is leveraged to synthesize a high-fidelity driving simulator and hence enable performance tests in virtual environments. Based on this practical experience, this paper also proposes a conceptual framework to support predictions based on real driving behavior.

==> _old_ml.tex <==

In the beginning, we provide an overview for the approach steps. Then in subsequent subsections, each approach step is detailed.


\begin{figure}[hbt]
	\centering
	\includegraphics[width=0.80\linewidth,height=3.2in]{figures/appr.png} 
	\caption{An Overview of the Proposed Approach. \label{fig3:appr}}
\end{figure}

\subsection{An Overview}
Figure~\ref{fig3:appr} shows a holistic view of the proposed approach. As shown, the approach consists of three main steps: features selection, pre-processing, and building prediction model. The approach takes, as an input, time series data for selected route(s) with specified number of features (such as, GPS information, curvature, slope, speed limit,  etc.). Unneeded features increase computation costs and degrade the generalization of prediction model. Therefore in the first step, we exclude unnecessary feature and keep only the important features for prediction. Then in the next step, the dataset undergoes the pre-processing step. After that, the data is divided into chunks: training data and testing data. the training data is used to build prediction model using supervised machine learning algorithm. The test data is used to evaluate the performance of the generated prediction model. The third step can be repeated many times with different ML algorithm each time until reach the best prediction model. Final the optimal prediction is saved to receive new route data for prediction purpose.

\subsection{Dataset Description}
\subsection{Feature Selection}
\subsection{Pre-processing}
\subsection{Building Prediction Model}



% sol1 - Neural Network (modello deterministico che non piace a darko)
% sol2 - Neural Network (type 1)
% sol3 - Neural Network (type 2)
